Method of Fundamental Solutions with Optimal Regularization Techniques for the Cauchy Problem of the Laplace Equation with Singular Points

The purpose of this study is to propose a high-accuracy and fast numerical method for the Cauchy problem of the Laplace equation. Our problem is directly discretized by the method of fundamental solutions (MFS). The Tikhonov regularization method stabilizes a numerical solution of the problem for given Cauchy data with high noises. The accuracy of the numerical solution depends on a regularization parameter of the Tikhonov regularization technique and some parameters of MFS. The L-curve determines a suitable regularization parameter for obtaining an accurate solution. Numerical experiments show that such a suitable regularization parameter coincides with the optimal one. Moreover, a better choice of the parameters of MFS is numerically observed. It is noteworthy that a problem whose solution has singular points can successfully be solved. It is concluded that the numerical method proposed in this paper is effective for a problem with an irregular domain, singular points, and the Cauchy data with high noises.

==> gamma.tex <==
%WinTpicVersion3.08
\unitlength 0.1in
\begin{picture}( 19.2000, 19.2000)(  0.0000,-19.2000)
% CIRCLE 2 1 3 0
% 4 960 960 1920 960 1920 960 1920 960
% 
\special{pn 8}%
\special{ar 960 960 960 960  0.0000000 0.0625000}%
\special{ar 960 960 960 960  0.1000000 0.1625000}%
\special{ar 960 960 960 960  0.2000000 0.2625000}%
\special{ar 960 960 960 960  0.3000000 0.3625000}%
\special{ar 960 960 960 960  0.4000000 0.4625000}%
\special{ar 960 960 960 960  0.5000000 0.5625000}%
\special{ar 960 960 960 960  0.6000000 0.6625000}%
\special{ar 960 960 960 960  0.7000000 0.7625000}%
\special{ar 960 960 960 960  0.8000000 0.8625000}%
\special{ar 960 960 960 960  0.9000000 0.9625000}%
\special{ar 960 960 960 960  1.0000000 1.0625000}%
\special{ar 960 960 960 960  1.1000000 1.1625000}%
\special{ar 960 960 960 960  1.2000000 1.2625000}%
\special{ar 960 960 960 960  1.3000000 1.3625000}%
\special{ar 960 960 960 960  1.4000000 1.4625000}%
\special{ar 960 960 960 960  1.5000000 1.5625000}%
\special{ar 960 960 960 960  1.6000000 1.6625000}%
\special{ar 960 960 960 960  1.7000000 1.7625000}%
\special{ar 960 960 960 960  1.8000000 1.8625000}%
\special{ar 960 960 960 960  1.9000000 1.9625000}%
\special{ar 960 960 960 960  2.0000000 2.0625000}%
\special{ar 960 960 960 960  2.1000000 2.1625000}%
\special{ar 960 960 960 960  2.2000000 2.2625000}%
\special{ar 960 960 960 960  2.3000000 2.3625000}%
\special{ar 960 960 960 960  2.4000000 2.4625000}%
\special{ar 960 960 960 960  2.5000000 2.5625000}%
\special{ar 960 960 960 960  2.6000000 2.6625000}%
\special{ar 960 960 960 960  2.7000000 2.7625000}%
\special{ar 960 960 960 960  2.8000000 2.8625000}%
\special{ar 960 960 960 960  2.9000000 2.9625000}%
\special{ar 960 960 960 960  3.0000000 3.0625000}%
\special{ar 960 960 960 960  3.1000000 3.1625000}%
\special{ar 960 960 960 960  3.2000000 3.2625000}%
\special{ar 960 960 960 960  3.3000000 3.3625000}%
\special{ar 960 960 960 960  3.4000000 3.4625000}%
\special{ar 960 960 960 960  3.5000000 3.5625000}%
\special{ar 960 960 960 960  3.6000000 3.6625000}%
\special{ar 960 960 960 960  3.7000000 3.7625000}%
\special{ar 960 960 960 960  3.8000000 3.8625000}%
\special{ar 960 960 960 960  3.9000000 3.9625000}%
\special{ar 960 960 960 960  4.0000000 4.0625000}%
\special{ar 960 960 960 960  4.1000000 4.1625000}%
\special{ar 960 960 960 960  4.2000000 4.2625000}%
\special{ar 960 960 960 960  4.3000000 4.3625000}%
\special{ar 960 960 960 960  4.4000000 4.4625000}%
\special{ar 960 960 960 960  4.5000000 4.5625000}%
\special{ar 960 960 960 960  4.6000000 4.6625000}%
\special{ar 960 960 960 960  4.7000000 4.7625000}%
\special{ar 960 960 960 960  4.8000000 4.8625000}%
\special{ar 960 960 960 960  4.9000000 4.9625000}%
\special{ar 960 960 960 960  5.0000000 5.0625000}%
\special{ar 960 960 960 960  5.1000000 5.1625000}%
\special{ar 960 960 960 960  5.2000000 5.2625000}%
\special{ar 960 960 960 960  5.3000000 5.3625000}%
\special{ar 960 960 960 960  5.4000000 5.4625000}%
\special{ar 960 960 960 960  5.5000000 5.5625000}%
\special{ar 960 960 960 960  5.6000000 5.6625000}%
\special{ar 960 960 960 960  5.7000000 5.7625000}%
\special{ar 960 960 960 960  5.8000000 5.8625000}%
\special{ar 960 960 960 960  5.9000000 5.9625000}%
\special{ar 960 960 960 960  6.0000000 6.0625000}%
\special{ar 960 960 960 960  6.1000000 6.1625000}%
\special{ar 960 960 960 960  6.2000000 6.2625000}%
% CIRCLE 0 0 3 0
% 4 960 960 1920 960 2240 960 2240 0
% 
\special{pn 20}%
\special{ar 960 960 960 960  5.6396842 6.2831853}%
% STR 2 0 3 0
% 3 1888 504 1888 584 2 0
% $\Gamma_1^{1/d}$
\put(18.8800,-5.8400){\makebox(0,0)[lb]{$\Gamma_1^{1/d}$}}%
% STR 2 0 3 0
% 3 232 1424 232 1504 2 0
% $\Gamma_2^{1/d}$
\put(2.3200,-15.0400){\makebox(0,0)[lb]{$\Gamma_2^{1/d}$}}%
% LINE 2 0 3 0
% 4 960 960 1728 384 1728 384 1728 384
% 
\special{pn 8}%
\special{pa 960 960}%
\special{pa 1728 384}%
\special{fp}%
\special{pa 1728 384}%
\special{pa 1728 384}%
\special{fp}%
% LINE 2 0 3 0
% 2 960 960 1920 960
% 
\special{pn 8}%
\special{pa 960 960}%
\special{pa 1920 960}%
\special{fp}%
% CIRCLE 2 0 3 0
% 4 960 960 1280 960 2400 960 2240 0
% 
\special{pn 8}%
\special{ar 960 960 320 320  5.6396842 6.2831853}%
% SARROW 2 0 3 1
% 2 1223 778 1216 768
% 
\special{pn 8}%
\special{pa 1224 778}%
\special{pa 1216 768}%
\special{fp}%
\special{sh 1}%
\special{pa 1216 768}%
\special{pa 1238 834}%
\special{pa 1248 812}%
\special{pa 1272 812}%
\special{pa 1216 768}%
\special{fp}%
% STR 2 0 3 0
% 3 1312 808 1312 888 2 0
% $2\pi/d$
\put(13.1200,-8.8800){\makebox(0,0)[lb]{$2\pi/d$}}%
\end{picture}%

